UW-SDF: Exploiting Hybrid Geometric Priors for Neural SDF Reconstruction from Underwater Multi-view Monocular Images

Due to the unique characteristics of underwater environments, accurate 3D reconstruction of underwater objects poses a challenging problem in tasks such as underwater exploration and mapping. Traditional methods that rely on multiple sensor data for 3D reconstruction are time-consuming and face challenges in data acquisition in underwater scenarios. We propose UW-SDF, a framework for reconstructing target objects from multi-view underwater images based on neural SDF. We introduce hybrid geometric priors to optimize the reconstruction process, markedly enhancing the quality and efficiency of neural SDF reconstruction. Additionally, to address the challenge of segmentation consistency in multi-view images, we propose a novel few-shot multi-view target segmentation strategy using the general-purpose segmentation model (SAM), enabling rapid automatic segmentation of unseen objects. Through extensive qualitative and quantitative experiments on diverse datasets, we demonstrate that our proposed method outperforms the traditional underwater 3D reconstruction method and other neural rendering approaches in the field of underwater 3D reconstruction.

==> sections/0_abstract_old.tex <==
\begin{abstract}

% This study introduces Water-SDF, a neural Signed Distance Fields (SDF) based framework for effective 3D reconstruction in complex underwater environments. Leveraging multi-view images, it addresses challenges such as underwater image enhancement and mono loss. To improve target reconstruction in cluttered scenes, a few-shot multi-view target segmentation strategy is proposed, utilizing a general-purpose segmentation model (SAM). The release of a benchmark dataset, including simulated and real underwater scenes, supports future research in underwater scene 3D reconstruction. Overall, this work offers a promising solution for accurate and robust underwater scene reconstruction.

% Accurate 3D reconstruction of underwater scenes is essential for the effective deployment of autonomous underwater vehicles (AUVs) and remotely operated vehicles (ROVs) in tasks such as mapping, inspection, and transportation. 
% This study introduces UW-SDF, a Neural Signed Distance Field (SDF) framework tailored for comprehensive 3D surface reconstruction in complex underwater environments. 
% Departing from previous NeRF-centric approaches, our focus is on surface reconstruction, utilizing SDF as an implicit representation of object surfaces. 
% To address challenges in scenarios with limited or textureless views, we propose a multi-view consistent underwater image enhancement strategy and a few-shot multi-view target segmentation strategy. 
% These innovations contribute to refined reconstruction, overcoming limitations associated with insufficient constraints. 
% The proposed framework and strategies showcase substantial improvements over existing methods, providing reliable and complete scene reconstruction results. 
% The released benchmark dataset, encompassing both simulated and real-world underwater scenes, establishes a standardized evaluation platform for single-view and multi-view underwater scene reconstruction. 
% This comprehensive contribution advances the field of underwater 3D reconstruction, offering a robust framework and innovative strategies that enhance the quality and accuracy of reconstructed underwater scenes.



Due to the unique characteristics of underwater environments, accurate 3D reconstruction of underwater objects poses a challenging problem in tasks such as underwater exploration and mapping. Traditional methods that rely on multiple sensor data for 3D reconstruction are time-consuming and face challenges in data acquisition in underwater scenarios.
We propose UW-SDF, a framework for reconstructing target objects from multi-view underwater images based on neural SDF. 
% It systematically explores the application of neural implicit representations in challenging underwater object reconstruction, significantly reducing the data collection difficulty in underwater 3D reconstruction. 
We introduce hybrid geometric cues to optimize the reconstruction process, markedly enhancing the quality and efficiency of neural SDF reconstruction. 
Additionally, addressing the challenge of consistent segmentation in multi-view images, we propose a novel few-shot multi-view target segmentation strategy using the general-purpose segmentation model (SAM), enabling rapid automatic segmentation of unseen objects. 
Through extensive qualitative and quantitative experiments on diverse datasets, we demonstrate that our proposed method outperforms the traditional underwater 3D reconstruction method and other neural rendering approaches in the field of underwater 3D reconstruction.


\end{abstract}

==> sections/1.tex <==
\section{INTRODUCTION}
\label{sec:intro}

%应用广泛
Reconstructing high-quality 3D underwater objects plays a crucial role in the deployment of autonomous underwater vehicles (AUVs) and remotely operated vehicles (ROVs) for mapping, inspection, and transportation tasks~\cite{zhang2021subsea, karapetyan2021human,islam2022svam}. 
% This functionality finds extensive applications in underwater archaeology, biological observation, and other fields. 
%Through underwater 3D reconstruction technology, researchers can gain in-depth insights into underwater topography, ecological environments, and cultural heritage, thereby providing robust support for marine ecological conservation and scientific research.

% However, due to the complexity of underwater environments, collecting data beneath the water surface is challenging. 
% The limited accessibility of underwater scenes, coupled with the difficulty in deploying and operating systems, often necessitates the involvement of skilled divers or specialized equipment. 
% Therefore, compared to acoustic methods, optical cameras, due to their passive, low-cost, and convenient nature, are widely used in underwater perception.
% Nevertheless, the absorption and scattering of light in water result in color distortion and image blurring, posing challenges for traditional visual methods in underwater environments. 
% Attempting 3D reconstruction directly using heavily scattered underwater images may lead to failures. Practical experience suggests that utilizing deep learning methods to enhance the imaging quality of underwater images can effectively eliminate interference from certain scattering media.

%光学方法挑战
However, collecting data in complex underwater environments is challenging and often necessitates the involvement of skilled divers or specialized equipment. Acoustic and optical sensors\cite{lyu2023structured,ding2023light,maccarone2023submerged,cong2021underwater,mcconnell2020fusing} are commonly used underwater, with optical cameras being widely applied due to their passive, cost-effective, and convenient nature in underwater perception. Nevertheless, the absorption and scattering of light in water can result in color distortion and blurring of images, posing challenges for traditional vision methods in underwater environments. The significant degradation of underwater images greatly affects the effectiveness of 3D reconstruction. Using deep learning methods to enhance the imaging quality of underwater images can mitigate the interference caused by scattering media. 

%nerf水下应用
Recently, the introduction of Neural Radiance Fields (NeRF) \cite{mildenhall2021nerf} technology has provided a new avenue for addressing tasks such as synthesizing novel perspectives and enhancing images in underwater scenes. Leveraging NeRF technology, these methods jointly estimate the parameters of scattering media through multiple views to eliminate the impact of scattering media on imaging. While these endeavors showcase the extensive potential of neural implicit methods in reconstructing underwater scenes, most efforts are limited to reconstructing two-dimensional images. In practical tasks such as mapping, exploration, and manipulation, three-dimensional geometric information is crucial. Therefore, our aim is to leverage 3D reconstruction technology to obtain the three-dimensional geometry of underwater targets and scenes.

Diverging from previous emphases on NeRF applications in underwater scenes, we emphasize surface reconstruction of underwater objects. 
We adopt the Signed Distance Field (SDF) as an implicit representation of object surfaces, utilizing the NeRF concept for parametric learning of this representation to achieve more refined surface reconstruction.

\input{figs/Head}

%神经隐式重建问题
Currently, surface reconstruction methods based on neural implicit representations have demonstrated favorable results in simple scenes with dense viewpoint sampling. However, in underwater environments, where views are limited or scenes contain large textureless areas, these methods face challenges. One key reason is that these models typically optimize using RGB reconstruction losses per pixel, making the quality of input multi-view images crucial. Given the substantial degradation of images captured underwater, relying solely on these images for construction may impose insufficient constraints, leading to suboptimal or unsuccessful reconstruction outcomes.

%采用混合线索
To address this limitation, we introduce a strategy that incorporates both 2D and 3D geometric cues to constrain the neural Signed Distance Function (SDF) reconstruction process. We utilize 2D foreground masks to mitigate the influence of cluttered backgrounds on the reconstruction target, and propose a novel few-shot multi-view automatic target segmentation strategy, achieving consistent segmentation of the target foreground in large, unstructured multi-view images. Additionally, we leverage depth and normal vectors as 3D geometric priors to optimize the training process, enhancing the restoration of details and textures.
% However, obtaining a consistent segmentation foreground of the target across a large and unordered set of multi-view images containing localized object information is challenging.

% Therefore, we propose a novel Few-Shot Multi-View Automatic Target Segmentation strategy. This approach requires annotating a small number of views and utilizes a General-Purpose Segmentation Model (SAM) to automatically segment unseen targets, swiftly generating masks tailored for the reconstruction task.

Therefore, the contributions of this study include:

\begin{itemize}

\item We introduce UW-SDF, a neural SDF-based 3D surface reconstruction framework that exploits hybrid 2D and 3D geometric cues to constrain the neural SDF reconstruction process, enabling the recovery of the geometric shape of target objects from underwater multi-view images.

\item We propose a novel few-shot multi-view target segmentation strategy that requires annotation of only a few views to leverage a general-purpose segmentation model (SAM) for automatic segmentation of unseen targets, enabling rapid acquisition of foreground masks.

\item We validate the proposed methods on multiple simulated and real datasets, demonstrating superior performance compared to other underwater 3D reconstruction methods, and provide a novel underwater object multi-view 3D reconstruction dataset, UW3D.



\end{itemize}

==> sections/2.tex <==
\section{RELATED WORK}
\input{figs/sdf}

\subsection{Neural implicit scene representations }

The emerging neural implicit field\cite{park2019deepsdf,wang2021neus,yariv2021volume} has gained extensive attention in the research community for its strong representation of three-dimensional geometry, powerful representation of radiation fields, and low memory usage. Neural representations based on implicit functions take the coordinates of a spatial point as input and output information about the object at that spatial point. In comparison to previous discrete representations such as voxels and point clouds\cite{paschalidou2018raynet,tulsiani2017multi}, the implicit function-based representation allows sampling the three-dimensional object representation at any spatial resolution, leading to outstanding performance in high-precision reconstruction.

Recently, some works have extended the application of Neural Radiance Fields (NeRF) to underwater scenes. Levy et al.\cite{levy2023seathru} developed a new rendering model for NeRF in scattering media based on the SeaThru underwater imaging model. They proposed an architecture suitable for learning underwater scene information and medium parameters and correctly rendered realistic synthetic novel view images in both simulated and real scenarios. Tianyi et al.\cite{zhang2023nerf} integrated underwater lighting effects into a volumetric rendering framework with end-to-end differentiability, recovering true-color (albedo) underwater images through joint learning of medium and neural scene representations.

However, the aforementioned NeRF-based works primarily focus on restoring the true color of underwater images and generating high-quality images from novel viewpoints. In contrast, our research emphasizes the surface reconstruction of underwater scenes. We employ SDF to implicitly represent the object's surface, leveraging the NeRF volumetric rendering concept to parameterize and learn this representation. With hybrid geometric priors, we achieve a more refined neural implicit surface reconstruction.


\subsection{Underwater 3D reconstruction}

Three-dimensional reconstruction is a technique that involves collecting multiple two-dimensional images or data points to create a three-dimensional model of an object or scene. Traditional underwater three-dimensional reconstruction methods typically rely on multisensor fusion technologies, including sonar, laser scanners, and cameras\cite{qi20223d,cui2021high}, to acquire multiple data sources for reconstructing underwater scenes. Currently, mainstream three-dimensional reconstruction techniques are primarily divided into image-based and laser scanner-based methods\cite{cui2021high}. In terms of cost-effectiveness, research by Ying Lo et al.\cite{lo2019comparison} indicates that laser scanning methods achieve comparable accuracy to image-based methods, but the image-based methods that automatically process data are more economical.

In recent years, with the continuous development of machine learning and deep learning, researchers have been exploring solutions to the challenges of underwater image three-dimensional reconstruction using techniques such as neural networks. Xiong et al.\cite{xiong2021wild} proposed a differentiable framework to reconstruct unknown dynamic water surfaces and scene geometry, optimizing through a specially constructed objective function.
%加案例

While multi-view three-dimensional reconstruction is widely used in the general three-dimensional reconstruction field, its application in underwater scenarios is limited due to the unique characteristics of underwater environments. Our approach demonstrates the potential of neural implicit surface reconstruction methods in the underwater reconstruction domain, providing a new and efficient solution for underwater reconstruction challenges.


\subsection{Target Segmentation}

Segmentation, as a fundamental task in computer vision, aims to understand images on a pixel-by-pixel basis. In recent years, researchers have explored various segmentation tasks, including semantic segmentation\cite{cheng2022masked,jain2023semask}, instance segmentation\cite{schult2023mask3d,wang2023cut}, and video object segmentation\cite{heo2023generalized,ke2023mask}. However, traditional segmentation methods often exhibit poor generalization, requiring separate training for specific tasks and struggling to extend to different tasks or new categories, especially in underwater scenarios.

Recently, researchers have proposed various large-scale vision models to address segmentation tasks, pre-trained on extensive mask data, demonstrating strong generalization capabilities. Among them, the SAM (Segment Anything Model)\cite{kirillov2023segment} model is a notable example, employing an end-to-end Transformer structure and achieving excellent results in object and region segmentation for various types of instructions. Meanwhile, parallel research\cite{jain2023oneformer,wang2023seggpt,zou2024segment} to SAM strives to tackle the challenges of image segmentation using different strategies and technologies. 
% Models like OneFormer\cite{jain2023oneformer}, SegGPT\cite{wang2023seggpt}, and SEEM\cite{zou2024segment} have achieved significant success in image segmentation tasks by introducing powerful context learning paradigms or leveraging multimodal references.

In the field of underwater 3D reconstruction, the data obtained in practical tasks often consist of an unordered set of multi-view images rather than videos, making video object segmentation methods unsuitable, achieving segmentation consistency across multiple views is a new challenge. Therefore, in our research, we propose a novel strategy that combines a general-purpose segmentation model. With just a few annotated key views, our approach achieves few-shot multi-view automatic object segmentation. By segmenting foreground target objects from background interference, it provides geometric clues for reconstruction, enhancing the quality of the reconstruction.

% It's worth noting that our segmentation strategy is training-free and versatile, providing better segmentation results for both in-domain and out-of-domain segmentation tasks. This offers a new approach to solving segmentation tasks for uncommon objects.



==> tables/results_real.tex <==
\begin{table}[t]
    \centering
    \caption{Quantitative comparisons of geometric reconstruction results on real-world scene}
    \begin{tabular}{cccc}
        \toprule
        \textbf{Method} & \textbf{Acc $\downarrow$} & \textbf{Comp $\downarrow$} & \textbf{Mean $\downarrow$} \\
        \midrule
        \textbf{Neus} & 3.94 & 7.26 & 5.60 \\
        \textbf{MonoSDF} & 1.62 & 2.60 & 2.11 \\
        \textbf{Ours} & 2.04 & 1.97 & 2.01 \\
        \bottomrule
    \end{tabular}
\end{table}
